The Zwicky Transient Facility Type Ia supernova survey: first data release and results

Type Ia supernovae (SNe~Ia) in the nearby Hubble flow are excellent distance indicators in cosmology. The Zwicky Transient Facility (ZTF) has observed a large sample of supernovae from an untargeted, rolling survey, reaching $20.8, 20.6, 20.3$ mag in $g$ $r$, and $i$-band, respectively. With a FoV of 47 sq.deg, ZTF discovered $>$ 3000 SNe~Ia in a little over 2.5 years. Here, we report on the sample of 761 spectroscopically classified SNe~Ia from the first year of operations (DR1). The sample has a median redshift $\bar z =$ 0.057, nearly a factor of two higher than the current low-$z$ sample. Our sample has a total of 934 spectra, of which 632 were obtained with the robotic SEDm on Palomar P60. We assess the potential for precision cosmology for a total of 305 SNe with redshifts from host galaxy spectra. The sample is already comparable in size to the entire combined literature low-$z$ anchor sample. The median first detection is 13.5 days before maximum light, about 10 days earlier than the median in the literature. Furthermore, six SNe from our sample are at $D_L < 80$ Mpc, for which host galaxy distances can be obtained in the JWST era, such that we have calibrator and Hubble flow SNe observed with the same instrument. In the entire duration of ZTF-I, we have observed nearly fifty SNe for which we can obtain calibrator distances, key for percent level distance scale measurements.

==> tables/parameter_priors_HD.tex <==
\begin{table}
\caption{Parameter priors for fitting the Year 1 magnitude-redshift relation}
\begin{tabular}{|c|c|c|c|}
\hline 
Parameter & Prior & Description \\
\hline
$a_{\rm B}$ & [-10, 10] & Hubble diagram \\
$\alpha$ & [0, 1] & Width-luminosity relation slope \\
$\beta$ & [0, 4] & Width-colour relation slope \\
$\sigma_{\rm int}$ & [0, 1] & Intrinsic scatter\\
\hline
\end{tabular}
\label{tab:prior_hd}
\end{table}

